Spawrious: A Benchmark for Fine Control of Spurious Correlation Biases

The problem of spurious correlations (SCs) arises when a classifier relies on non-predictive features that happen to be correlated with the labels in the training data. For example, a classifier may misclassify dog breeds based on the background of dog images. This happens when the backgrounds are correlated with other breeds in the training data, leading to misclassifications during test time. Previous SC benchmark datasets suffer from varying issues, e.g., over-saturation or only containing one-to-one (O2O) SCs, but no many-to-many (M2M) SCs arising between groups of spurious attributes and classes. In this paper, we present \benchmark-\{O2O, M2M\}-\{Easy, Medium, Hard\}, an image classification benchmark suite containing spurious correlations between classes and backgrounds. To create this dataset, we employ a text-to-image model to generate photo-realistic images and an image captioning model to filter out unsuitable ones. The resulting dataset is of high quality and contains approximately 152k images. Our experimental results demonstrate that state-of-the-art group robustness methods struggle with \benchmark, most notably on the Hard-splits with none of them getting over $70\%$ accuracy on the hardest split using a ResNet50 pretrained on ImageNet. By examining model misclassifications, we detect reliances on spurious backgrounds, demonstrating that our dataset provides a significant challenge.

==> tables/m2m_combinations.tex <==
\begin{table*}
        \centering
        \resizebox{\textwidth}{!}{
        \begin{tabular}{|c|ccc|ccc|ccc|}
        \toprule
        \bf \multirow{2}{*}{Class} & \multicolumn{3}{c|}{\bf Many-To-Many Easy} &  \multicolumn{3}{c|}{\bf Many-To-Many Medium}  & \multicolumn{3}{c|}{\bf Many-To-Many Hard}\\
        \cmidrule{2-10}
        & \bf Env 1 & \bf Env 2 & \bf Test & \bf Env 1 & \bf Env 2 & \bf Test & \bf Env 1 & \bf Env 2 & \bf Test   \\
        \hline
        Bulldog & 100\% Dirt & 100\% Jungle & 50\% Snow 50\% Beach 
        & 100\% Desert & 100\% Mountain & 50\% Dirt 50\% Jungle 
        & 100\% Beach & 100\% Snow & 50\% Desert 50\% Mountain  \\
        
        Dachshund & 100\% Jungle & 100\% Dirt & 50\% Snow 50\% Beach 
        & 100\% Mountain & 100\% Desert & 50\% Dirt 50\% Jungle 
        & 100\% Beach & 100\% Snow & 50\% Desert 50\% Mountain \\

        Labrador & 100\% Snow & 100\% Beach & 50\% Dirt 50\% Jungle 
        & 100\% Dirt & 100\% Jungle & 50\% Desert 50\% Mountain 
        & 100\% Mountain & 100\% Desert & 50\% Beach 50\% Snow \\

        Corgi & 100\% Beach & 100\% Snow & 50\% Dirt 50\% Jungle 
        & 100\% Jungle & 100\% Dirt & 50\% Desert 50\% Mountain 
        & 100\% Mountain & 100\% Desert & 50\% Beach 50\% Snow  \\

        \bottomrule
        \end{tabular}}

     \caption{\textbf{Data combinations in \benchmark-\{O2O\}-\{Easy, Medium, Difficult\},}}
     \label{tab:results_new_archs}
\end{table*}
